Quantitative Verification of Neural Networks And its Security Applications

Neural networks are increasingly employed in safety-critical domains. This has prompted interest in verifying or certifying logically encoded properties of neural networks. Prior work has largely focused on checking existential properties, wherein the goal is to check whether there exists any input that violates a given property of interest. However, neural network training is a stochastic process, and many questions arising in their analysis require probabilistic and quantitative reasoning, i.e., estimating how many inputs satisfy a given property. To this end, our paper proposes a novel and principled framework to quantitative verification of logical properties specified over neural networks. Our framework is the first to provide PAC-style soundness guarantees, in that its quantitative estimates are within a controllable and bounded error from the true count. We instantiate our algorithmic framework by building a prototype tool called NPAQ that enables checking rich properties over binarized neural networks. We show how emerging security analyses can utilize our framework in 3 concrete point applications: quantifying robustness to adversarial inputs, efficacy of trojan attacks, and fairness/bias of given neural networks.

==> paper-dotfiles/paper-dot2tex-fig1.tex <==
%%
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{1.0,1.0,1.0};
  \pgfsetstrokecolor{strokecol}
  \definecolor{fillcol}{rgb}{1.0,1.0,1.0};
  \pgfsetfillcolor{fillcol}
  \filldraw (0.0bp,0.0bp) -- (0.0bp,306.0bp) -- (428.0bp,306.0bp) -- (428.0bp,0.0bp) -- cycle;
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{1.0,1.0,1.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,46.0bp) -- (8.0bp,206.0bp) -- (132.0bp,206.0bp) -- (132.0bp,46.0bp) -- cycle;
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{1.0,1.0,1.0};
  \pgfsetstrokecolor{strokecol}
  \definecolor{fillcol}{rgb}{1.0,1.0,1.0};
  \pgfsetfillcolor{fillcol}
  \filldraw (0.0bp,0.0bp) -- (0.0bp,306.0bp) -- (428.0bp,306.0bp) -- (428.0bp,0.0bp) -- cycle;
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{1.0,1.0,1.0};
  \pgfsetstrokecolor{strokecol}
  \draw (296.0bp,100.0bp) -- (296.0bp,152.0bp) -- (420.0bp,152.0bp) -- (420.0bp,100.0bp) -- cycle;
\end{scope}
  \node (rank2) at (214.0bp,288.0bp) [] {$$};
  \coordinate (rank1) at (70.0bp,234.0bp);
  \node (O) at (358.0bp,126.0bp) [vars] {$y$};
  \node (v1) at (214.0bp,234.0bp) [vars] {$v_1$};
  \node (v2) at (214.0bp,180.0bp) [vars2] {$v_2$};
  \node (v3) at (214.0bp,126.0bp) [vars2] {$v_3$};
  \node (v4) at (214.0bp,72.0bp) [vars2] {$v_4$};
  \node (v5) at (214.0bp,18.0bp) [vars] {$v_5$};
  \node (x2) at (70.0bp,126.0bp) [n] {$x_2$};
  \node (x3) at (70.0bp,72.0bp) [n] {$x_3$};
  \node (x1) at (70.0bp,180.0bp) [n] {$x_1$};
  \draw [->] (v5) ..controls (260.78bp,53.084bp) and (300.59bp,82.939bp)  .. node {$$} (O);
  \draw [->] (x1) ..controls (110.94bp,133.95bp) and (162.09bp,76.396bp)  .. node {$$} (v5);
  \draw [->] (x2) ..controls (116.78bp,161.08bp) and (156.59bp,190.94bp)  .. node {$$} (v1);
  \draw [->] (x1) ..controls (124.87bp,200.57bp) and (148.23bp,209.34bp)  .. node {$$} (v1);
  \draw [red,->,dashed] (x1) ..controls (116.78bp,144.92bp) and (156.59bp,115.06bp)  .. node {$$} (v4);
  \draw [red,->,dashed] (x2) ..controls (124.87bp,146.57bp) and (148.23bp,155.34bp)  .. node {$$} (v2);
  \draw [red,->,dashed] (x3) ..controls (124.87bp,92.575bp) and (148.23bp,101.34bp)  .. node {$$} (v3);
  \draw [red,->,dashed] (v3) ..controls (276.31bp,126.0bp) and (284.94bp,126.0bp)  .. node {$$} (O);
  \draw [->] (v1) ..controls (260.78bp,198.92bp) and (300.59bp,169.06bp)  .. node {$$} (O);
  \draw [red,->,dashed] (x2) ..controls (132.31bp,126.0bp) and (140.94bp,126.0bp)  .. node {$$} (v3);
  \draw [red,->,dashed] (x3) ..controls (116.78bp,107.08bp) and (156.59bp,136.94bp)  .. node {$$} (v2);
  \draw [red,->,dashed] (x1) ..controls (124.87bp,159.43bp) and (148.23bp,150.66bp)  .. node {$$} (v3);
  \draw [->] (x3) ..controls (124.87bp,51.425bp) and (148.23bp,42.664bp)  .. node {$$} (v5);
  \draw [red,->,dashed] (v4) ..controls (268.87bp,92.575bp) and (292.23bp,101.34bp)  .. node {$$} (O);
  \draw [red,->,dashed] (x2) ..controls (124.87bp,105.43bp) and (148.23bp,96.664bp)  .. node {$$} (v4);
  \draw [->] (x3) ..controls (110.94bp,118.05bp) and (162.09bp,175.6bp)  .. node {$$} (v1);
  \draw [red,->,dashed] (x1) ..controls (132.31bp,180.0bp) and (140.94bp,180.0bp)  .. node {$$} (v2);
  \draw [red,->,dashed] (v2) ..controls (268.87bp,159.43bp) and (292.23bp,150.66bp)  .. node {$$} (O);
  \draw [red,->,dashed] (x3) ..controls (132.31bp,72.0bp) and (140.94bp,72.0bp)  .. node {$$} (v4);
  \draw [->] (x2) ..controls (116.78bp,90.916bp) and (156.59bp,61.061bp)  .. node {$$} (v5);
%

==> tables/arch-setup-acc.tex <==


\caption{BNN architecture description and accuracy (Acc) 
over MNIST dataset scaled to 10$\times$10 images and UCI Adult datasets.}\label{tab:setup}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{c|lll|cc}
\toprule
  \textbf{Name} & \multicolumn{3}{c|}{\textbf{Arch (Block \& No. of Neurons)}} &
  \textbf{Acc MNIST (\%)} & \textbf{Acc Adult (\%)} \\ 
\midrule 
  \textbf{ARCH$_1$} & BLK$_1$(100)& & & 76 & 76 \\ 
  \textbf{ARCH$_2$} & BLK$_1$(50)& BLK$_2$(20) & & 79 & 81 \\ 
  \textbf{ARCH$_3$} & BLK$_1$(100)&BLK$_2$(50) & & 80 & 80 \\ 
  \textbf{ARCH$_4$} & BLK$_1$(200)&BLK$_2$(100) & BLK$_3$(100) & 88 & 80 \\ \bottomrule
\end{tabular}%
}


==> tables/arch-setup.tex <==
\begin{table}[]
\centering
\caption{BNN architecture description}\label{tab:setup}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{c|lll}
\toprule
  \textbf{Name} & \multicolumn{3}{c|}{\textbf{Arch (Block \& No. of Neurons)}}
  \\ \hline
  \textbf{ARCH$_1$} & BLK$_1$(100)& & \\ 
  \textbf{ARCH$_2$} & BLK$_1$(50)& BLK$_2$(20) &  \\ 
  \textbf{ARCH$_3$} & BLK$_1$(100)&BLK$_2$(50) &  \\ 
  \textbf{ARCH$_4$} & BLK$_1$(200)&BLK$_2$(100) & BLK$_3$(100)  \\ \bottomrule
\end{tabular}%
}
\end{table}


==> tables/mnist-trojan_dist.tex <==
\begin{table}[]
\centering
\caption{Estimated difference of class distributions between a plain BNN without trojan attack  for $10 × 10$ and the trojaned models trained for epoch 1, 10 and 30 on 4 architectures ARCH$_{1..4}$. Column `TC' represents the target class of the trojan attack.}
\label{tab:trojan_dist}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Arch}} & \multirow{2}{*}{\textbf{TC}} & \multicolumn{3}{c|}{\textbf{KL Divergence}} \\ \cline{3-5} 
 &  & \textbf{Epoch=1} & \textbf{Epoch=10} & \textbf{Epoch=30} \\ \hline
\multirow{5}{*}{\textbf{ARCH$_1$}}
 & \textbf{0} & 0.0194 & 0.0546 & 0.0609 \\ \cline{2-5} 
 & \textbf{1} & 0.0646 & 0.0420 & 0.0605 \\ \cline{2-5} 
 & \textbf{4} & 0.0646 & 0.0420 & 0.0605 \\ \cline{2-5} 
 & \textbf{5} & 0.0691 & 0.0620 & 0.0688 \\ \cline{2-5} 
 & \textbf{9} & 0.0667 & 0.0549 & 0.0715 \\ \hline
\multirow{5}{*}{\textbf{ARCH$_2$}}
 & \textbf{0} & 0.0671 & 0.0299 & 0.0227 \\ \cline{2-5} 
 & \textbf{1} & 0.0658 & 0.0656 & 0.0635 \\ \cline{2-5} 
 & \textbf{4} & 0.0687 & 0.0599 & 0.0300 \\ \cline{2-5} 
 & \textbf{5} & 0.0653 & 0.0522 & 0.0550 \\ \cline{2-5} 
 & \textbf{9} & 0.0706 & 0.0508 & 0.0615 \\ \hline
\multirow{5}{*}{\textbf{ARCH$_3$}}
 & \textbf{0} & 0.0449 & 0.0426 & 0.0473 \\ \cline{2-5} 
 & \textbf{1} & 0.0614 & 0.0472 & 0.0636 \\ \cline{2-5} 
 & \textbf{4} & 0.0606 & 0.0593 & 0.0559 \\ \cline{2-5} 
 & \textbf{5} & 0.0625 & 0.0529 & 0.0585 \\ \cline{2-5} 
 & \textbf{9} & 0.0700 & 0.0717 & 0.0545 \\ \hline
\multirow{5}{*}{\textbf{ARCH$_4$}}
 & \textbf{0} & 0.0702 & 0.0664 & 0.0596 \\ \cline{2-5} 
 & \textbf{1} & 0.0601 & 0.0726 & 0.0646 \\ \cline{2-5} 
 & \textbf{4} & 0.0664 & 0.0670 & 0.0681 \\ \cline{2-5} 
 & \textbf{5} & 0.0698 & 0.0608 & 0.0627 \\ \cline{2-5} 
 & \textbf{9} & 0.0654 & 0.0665 & 0.0643 \\ \hline
\end{tabular}
\end{table}

==> tables/soa_table.tex <==
\begin{table*}[htbp!]
\caption{
Related Work on Verifying Neural Networks (Robustness Property). 
Column $1-2$ represent the approach details. 
Column $4$ denotes the \textit{Completeness} quality
to signify if the verification method is
exhaustive: it either proves that the verified property holds or it finds a
counter-example where the property does not hold ($\boldcheckmark$ for complete,
\xmark~ for incomplete procedures). 
Column$5$ represents the \textit{Complexity}, a $\boldcheckmark$ 
denotes there is an analysis on the complexity and $\xmark~$ 
means the analysis is incomplete. 
Column $6$ represents \textit{ML Integration} 
to signify whether the results can be fed back in the training
so that the model incorporates these results and becomes safer -- a $\boldcheckmark$
if so, otherwise \xmark~. Column $7$ for \textit{Generality}
describes the types of networks the approach can handle.
}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Work} & \multicolumn{1}{c|}{\textbf{Technique}} & \textbf{\begin{tabular}[c]{@{}c@{}}Tool\\ available\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Comple\\-teness\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Comp\\-lexity\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ML\\ Integr\end{tabular}} & \textbf{Generality} \\ \hline
Ehlers~\cite{ehlers2017formal} & customized SMT solving &
  \href{https://github.com/progirep/planet}{planet} & \boldcheckmark & \xmark &  \xmark & ReLU and max pool layers \\ \hline
Katz et al.~\cite{katz2017reluplex}  & customized SMT solving &
  \href{https://github.com/guykatzz/ReluplexCav2017}{Reluplex} & \boldcheckmark & \xmark  & \xmark  & ReLU layers \\ \hline
Wang et al..~\cite{wang2018intervals} & symbolic intervals &
  \href{https://github.com/tcwangshiqi-columbia/ReluVal}{ReluVal} & \boldcheckmark &
  \boldcheckmark & \xmark  & ReLU layers \\ \hline
  Gehr et al.~\cite{gehr2018ai2} & abstract interpretation &
  \href{https://github.com/eth-sri/eran}{ERAN} & \boldcheckmark &  \xmark  &  \xmark & ReLU, conv and max pool layers \\ \hline
Ruan et al.~\cite{ruan2018ijcai} & reachability analysis &
  \href{https://github.com/TrustAI/DeepGO}{DeepGO} & \xmark & \boldcheckmark  & \xmark  & piecewise linear \\ \hline
Raghunathan et al.~\cite{raghunathan2018certified} & convex optimization & -- & \xmark & \xmark & \boldcheckmark &
  only one non-linear  \\ \hline
Kolter et al.~\cite{wong2018provable} & convex optimization & -- & \xmark & \xmark & \boldcheckmark  &
  piecewise linear  \\ \hline
Narodytska et al.~\cite{narodytska2017verifying} & SAT solving & -- & \boldcheckmark  & \xmark & \xmark  & binarized neural networks \\ \hline
Dvijotham et al.~\cite{dvijotham2018dual} & convex optimization & -- & \xmark & \boldcheckmark &
  \boldcheckmark & arbitrary NNs \\ \hline
\end{tabular}
  }
\label{table:soa}
\end{table*}

